Improved summations of $n$-point correlation functions of projected entangled-pair states

Numerical treatment of two dimensional strongly-correlated systems is both extremely challenging and of fundamental importance. Infinite projected entangled-pair states (PEPS), a class of tensor networks, have demonstrated cutting-edge performance for ground state calculations, working directly in the thermodynamic limit. Furthermore, in recent years the application of PEPS has been extended to also low-lying excited states, using an ansatz that targets quasiparticle states above the ground state with high accuracy. A major technical challenge for those simulations is the accurate evaluation of summations of two- and three-point correlation functions with reasonable computational cost. In this work, we show how a reformulation of $n$-point functions in the context of PEPS leads to extra contributions to the results that prove to play an important role. Benchmarks for the frustrated $J_1-J_2$ Heisenberg model illustrate the improved precision, efficiency and stability of the simulations compared to previous approaches. Leveraging automatic differentiation to generate the most tedious and error-prone parts of the computation, the straightforward implementation presented here is a step towards broader adoption of the PEPS excitation ansatz in future applications.

==> include/tikz_intro.tex <==
% \tikzstyle{HB} = [draw=blue, line width=0.05cm, fill=blue, minimum height=0.75cm, minimum width=0.75cm, rounded corners=0.1cm, text=blue]
\tikzstyle{HB} = [preaction={fill, blue}, pattern=flexible hatch, pattern color=red, hatch distance=0.3cm, hatch thickness=0.05cm, line width=0.05cm, minimum height=0.75cm, minimum width=0.75cm, rounded corners=0.1cm, text=white, draw=blue]
% \tikzstyle{HB} = [preaction={fill, blue}, pattern=custom north east lines, pattern color=red, line width=0.05cm, minimum height=0.75cm, minimum width=0.75cm, rounded corners=0.1cm, text=white, draw=blue]

\tikzstyle{N} = [draw=grey, line width=0.05cm, fill=white, minimum height=0.75cm, minimum width=0.75cm, rounded corners=0.1cm, text=grey]
\tikzstyle{H} = [preaction={fill, white}, pattern=flexible hatch, pattern color=red, hatch distance=0.3cm, hatch thickness=0.05cm, draw=red, line width=0.05cm, minimum height=0.75cm, minimum width=0.75cm, rounded corners=0.1cm, text=red, text opacity=0]
% \tikzstyle{H} = [preaction={fill, white}, pattern=custom north east lines, pattern color=red, draw=red, line width=0.05cm, minimum height=0.75cm, minimum width=0.75cm, rounded corners=0.1cm, text=red, text opacity=0]
\tikzstyle{B} = [draw=blue, line width=0.05cm, fill=blue, minimum height=0.75cm, minimum width=0.75cm, rounded corners=0.1cm, text opacity=1, text=white]
\tikzstyle{Bd} = [draw=darkblue, line width=0.05cm, fill=darkblue, minimum height=0.75cm, minimum width=0.75cm, rounded corners=0.1cm, text opacity=1, text=white]
\tikzstyle{BBd} = [preaction={fill, darkblue}, pattern=flexible hatch, pattern color=blue, hatch distance=0.3cm, hatch thickness=0.05cm, draw=blue, line width=0.05cm, minimum height=0.75cm, minimum width=0.75cm, rounded corners=0.1cm, text opacity=1, text=white]

\tikzstyle{tensor} = [draw=grey, line width=0.05cm, fill=white, minimum height=0.4cm, circle, inner sep=0cm]
\tikzstyle{tensorxin} = [draw=grey, line width=0.05cm, fill=white, minimum height=0.4cm, circle, text=red, inner sep=0cm, fill opacity=0, text opacity=1, draw opacity=0]
\tikzstyle{tensorx} = [draw=red, line width=0.05cm, fill=white, minimum height=0.4cm, circle, text=red, inner sep=0cm]
\tikzstyle{tensorb} = [draw=blue, line width=0.05cm, fill=blue, minimum height=0.4cm, circle, text=blue, inner sep=0cm]
\tikzstyle{tensorbd} = [draw=darkblue, line width=0.05cm, fill=darkblue, minimum height=0.4cm, circle, text=darkblue, inner sep=0cm]
\tikzstyle{tensorbbd} = [preaction={fill, darkblue}, pattern=flexible hatch, pattern color=blue, hatch distance=0.3cm, hatch thickness=0.05cm, draw=blue, line width=0.05cm, minimum height=0.4cm, circle, text=darkblue, inner sep=0cm]
\tikzstyle{tensorxb} = [draw=blue, line width=0.05cm, fill=blue, minimum height=0.4cm, circle, text=red, inner sep=0cm]

\tikzstyle{proj} = [regular polygon,regular polygon sides=3, shape border rotate=180, draw=black, fill=black, line width=0.05cm,inner sep=0cm, minimum size=0.45cm, rounded corners=0.05cm, text=green, text opacity=0]
% \tikzstyle{Hconnect} = [draw=red, line width=0.05cm, dashed, fill=red, inner sep=0cm, minimum width=1.2cm, minimum height=0.2cm, rounded corners=0.1cm, text=blue, fill opacity=0, draw opacity=1]
\tikzstyle{Hconnecth} = [draw=red, line width=0.00cm, fill=red, inner sep=0cm, minimum width=1.2cm, minimum height=0.25cm, rounded corners=0.0cm, text=blue, fill opacity=0.7, draw opacity=0]
\tikzstyle{Hconnectv} = [draw=red, line width=0.00cm, fill=red, inner sep=0cm, minimum width=0.25cm, minimum height=1.2cm, rounded corners=0.0cm, text=blue, fill opacity=0.7, draw opacity=0]

\tikzstyle{T} = [minimum width=0.4cm, rounded corners=0.15cm, inner sep=0cm]
\tikzstyle{Th} = [minimum height=0.4cm, rounded corners=0.15cm, inner sep=0cm]
\tikzstyle{Ch} = [minimum width=1.65cm]
\tikzstyle{Cv} = [minimum height=1.65cm]
\tikzstyle{TTh} = [minimum width=1.60cm]
\tikzstyle{TTv} = [minimum height=1.60cm]
% \tikzstyle{doubline} = [line width=0.02cm, double, double distance=0.075cm]
 

% Pattern
\tikzset{
  hatch distance/.store in=\hatchdistance,
  hatch distance=10pt,
  hatch thickness/.store in=\hatchthickness,
  hatch thickness=2pt
}

% Projector
\tikzset{
  projector/.pic={
    \node[proj, name=proj] at (0.5,-0.75) {};
    \draw[line width=0.1cm] (0,-0.4) to[out=270,in=90] ($(proj)+(-0.05,0.12)$);
    \draw[doubline] (1,-0.4) to[out=270,in=90] ($(proj)+(0.05,0.12)$);
    \draw[line width=0.1cm] ($(proj)+(0,-0.12)$) -- ($(proj)+(0,-0.35)$);
    \node[proj] at (proj) {};
}}
\tikzset{
  projector up/.pic={
    \node[proj, name=proj, shape border rotate=0] at (0.5,0.75) {};
    \draw[line width=0.1cm] (0,0.4) to[out=90,in=270] ($(proj)+(-0.05,-0.12)$);
    \draw[doubline] (1,0.4) to[out=90,in=270] ($(proj)+(0.05,-0.12)$);
    \draw[line width=0.1cm] ($(proj)+(0,0.12)$) -- ($(proj)+(0,0.35)$);
    \node[proj, shape border rotate=0] at (proj) {};
}}
\tikzset{
  projector up high/.pic={
    \node[proj, name=proj, shape border rotate=0] at (0.5,1.75) {};
    \draw[line width=0.1cm] (0,1.4) to[out=90,in=270] ($(proj)+(-0.05,-0.12)$);
    \draw[doubline] (1,1.4) to[out=90,in=270] ($(proj)+(0.05,-0.12)$);
    \draw[line width=0.1cm] ($(proj)+(0,0.12)$) -- ($(proj)+(0,0.35)$);
    \node[proj, shape border rotate=0] at (proj) {};
}}

\tikzset{doubline/.style={% \tikzstyle is deprecated
    preaction={
      draw=black,
      double distance between line centers=0.075cm,
      line width=0.04cm,
      shorten >=0pt,
      shorten <=0pt,
    },
    draw=white,
    line width=0.075cm,
    shorten >=-.1pt,
    shorten <=-.1pt,
  }}

% % defining the new dimensions and parameters
% \newlength{\hatchspread}
% \newlength{\hatchthickness}
% \newlength{\hatchshift}
% \newcommand{\hatchcolor}{}
% % declaring the keys in tikz
% \tikzset{hatchspread/.code={\setlength{\hatchspread}{#1}},
%          hatchthickness/.code={\setlength{\hatchthickness}{#1}},
%          hatchshift/.code={\setlength{\hatchshift}{#1}},% must be >= 0
%          hatchcolor/.code={\renewcommand{\hatchcolor}{#1}}}
% % setting the default values
% \tikzset{hatchspread=5pt,
%          hatchthickness=0.8pt,
%          hatchshift=0pt,% must be >= 0
%          hatchcolor=black}
% \pgfdeclarepatternformonly[\hatchspread,\hatchthickness,\hatchshift,\hatchcolor]% variables
%    {custom north east lines}% name
%    {\pgfqpoint{\dimexpr-2\hatchthickness}{\dimexpr-2\hatchthickness}}% lower left corner
%    {\pgfqpoint{\dimexpr\hatchspread+2\hatchthickness}{\dimexpr\hatchspread+2\hatchthickness}}% upper right corner
%    {\pgfqpoint{\dimexpr\hatchspread}{\dimexpr\hatchspread}}% tile size
%    {% shape description
%     \pgfsetlinewidth{\hatchthickness}
%     \pgfpathmoveto{\pgfqpoint{\dimexpr\hatchshift-0.15pt}{-0.15pt}}
%     \pgfpathlineto{\pgfqpoint{\dimexpr\hatchspread+0.15pt}{\dimexpr\hatchspread-\hatchshift+0.15pt}}
%     \ifdim \hatchshift > 0pt
%       \pgfpathmoveto{\pgfqpoint{-0.15pt}{\dimexpr\hatchspread-\hatchshift-0.15pt}}
%       \pgfpathlineto{\pgfqpoint{\dimexpr\hatchshift+0.15pt}{\dimexpr\hatchspread+0.15pt}}
%     \fi
%     \pgfsetstrokecolor{\hatchcolor}
% %    \pgfsetdash{{1pt}{1pt}}{0pt}% dashing cannot work correctly in all situation this way
%     \pgfusepath{stroke}
%    }

